Understanding the Impact of Model Incoherence on Convergence of Incremental SGD with Random Reshuffle

Although SGD with random reshuffle has been widely-used in machine learning applications, there is a limited understanding of how model characteristics affect the convergence of the algorithm. In this work, we introduce model incoherence to characterize the diversity of model characteristics and study its impact on convergence of SGD with random reshuffle under weak strong convexity. Specifically, minimizer incoherence measures the discrepancy between the global minimizers of a sample loss and those of the total loss and affects the convergence error of SGD with random reshuffle. In particular, we show that the variable sequence generated by SGD with random reshuffle converges to a certain global minimizer of the total loss under full minimizer coherence. The other curvature incoherence measures the quality of condition numbers of the sample losses and determines the convergence rate of SGD. With model incoherence, our results show that SGD has a faster convergence rate and smaller convergence error under random reshuffle than those under random sampling, and hence provide justifications to the superior practical performance of SGD with random reshuffle.

==> config.tex <==
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem*{definition*}{Definition} 
\newtheorem{example}[definition]{Example} 
	
\theoremstyle{plain}
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}[definition]{Proposition}
\newtheorem{corollary}[definition]{Corollary}
\newtheorem{assumption}[definition]{Assumption}
\newtheorem{condition}[definition]{Condition}
\newtheorem{exercise}[definition]{Exercise}
  
\newtheorem*{theorem*}{Theorem}
\newtheorem*{lemma*}{Lemma}
\newtheorem*{proposition*}{Proposition}
\newtheorem{corollary*}{Corollary}   
\newtheorem{assumption*}{Assumption}
\newtheorem{condition*}{Condition}
\newtheorem{exercise*}{Exercise}
	
\theoremstyle{remark}
\newtheorem*{remark}{Remark}

==> extentions.tex <==
\subsection{Discussion on Sampling Scheme}


\subsection{Optimal Batch Size}
\begin{definition}[batch-model incoherence] Assume the dataset with $n$ observations is divided into $m$ mini-batches ($b_1, \dots, b_m$).Then $\frac{n}{m}$ is the batch size and the batch-model incoherence of the $i$-th mini-batch is defined as 
	$$\epsilon_{b_i} = \sup_{\theta \in \Theta} \frac{m}{n}\sum_{j \in b_i} l_j(\theta) - \frac{m}{n}( \sum_{j \in b_i} l_j )^\ast. $$
\end{definition}
\begin{remark}
	For gradient decent, it is easy to see $\epsilon = 0$.
\end{remark}

\begin{thm}\label{batchsize1}
	Let $b$ be a given mini-batch and $\epsilon_b$ be the batch-model incoherence on the batch $b$. Then 
	$$\epsilon_b \leq (\sum_{j\in b } \epsilon_i) \cdot \frac{m}{n}.$$
\end{thm}

\begin{example}
	Under strongly convex assumption  
	$$\epsilon_b \leq (\sum_{j \in b} \epsilon_j- \sum_{j \in b}\alpha_j \| \theta_b - \theta_j^\ast \|^2)\cdot \frac{m}{n}.$$
\end{example}

\begin{lemma}[Batch $\alpha$-diverse]\label{lemma: batch_alpha}
	For any $\theta \notin \bigcup_{i=1}^n \Theta_i^*$, there exists $\alpha \le 1$ such that
	\begin{align*}
	f(\theta) - \ell_{b(j)}(\theta)  \leq &\alpha \left( f(\theta) - f^\ast \right) + \frac{1}{m}\sum_{i=1}^m (\ell_{b(i)}^\ast+\epsilon_{b(i)}) - \ell_{b(j)}(\theta). 
	\end{align*}
\end{lemma}
$K=mB$.
\begin{thm} 
	Let \Cref{assum: exist} and \ref{assum: f} hold for the problem (P). Apply SGD with cyclic-types of sampling schemes and learning rate $\eta<\frac{2}{L}$ to solve the problem (P). Then, the average of the total loss along the optimization path $\{\theta_k\}_k$ satisfies
	\begin{align*}
	\frac{1}{K}\sum_{k=0}^{K-1}  f( \theta_{k}) - f^\ast  \leq \frac{L\dist_\Theta^2(\theta_{0})}{2K(1-\alpha)} + \frac{\sum_{i=1}^m \epsilon_i}{m(1-\alpha)}.
	\end{align*}
\end{thm}

If all loss are $\mu_i$ r.s.c

\subsection{Effect of Sampling Scheme}
Sampling scheme may influence the batch model incoherence.  
\begin{definition} Let $\sigma \in \{1,\dots, n\}^n$. Assume $n$ observations is divided into $m$ mini-batches ($b_1, \dots, b_m$). The batch-model incoherence of the $i$-th mini-batch corresponding to the permutation $\sigma$ is defined as 
	$$\epsilon_{b_i}(\sigma) = \sup_{\theta \in \Theta} \frac{m}{n}\sum_{j \in b_i} l_{\sigma(j)}(\theta) - \frac{m}{n}( \sum_{j \in b_i} l_{\sigma(j)} )^\ast. $$
\end{definition}
Given $m$ mini-batches $\{ b_1, \dots, b_m \}$, define $\mathcal{L}: S_n \to \RR_+$ as
\begin{align*}
\mathcal{L}: \sigma \mapsto \frac{1}{m}\sum_{i=1}^m \epsilon_{b_i}(\sigma).
\end{align*} 
Let $\sigma^\ast := \argmin_{\sigma \in S_n} \mathcal{L}$. \textbf{Question:} Is it the best choice?



==> header.tex <==

% BASIC PACKAGES %

\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{fullpage}
%\usepackage{tikz} %画交换图
%\usepackage{amscd} %画交换图
\usepackage{comment} %大段注释
\usepackage{xcolor}
\usepackage{soul}
\usepackage{enumerate}
\usepackage{graphicx}
\usepackage{float} %插入图片
\usepackage{ulem} %波浪线 
\usepackage{tcolorbox}

 
% EMPHASIZE BOX %

\usepackage{empheq}
\newcommand{\widefbox}[1]{\fbox{\hspace{0.33in}#1\hspace{0.33in}}}

 



